Addressing Systematics in the Traceback Age of the $\beta$ Pictoris Moving Group

We characterize the impact of several sources of systematic errors on the computation of the traceback age of the $\beta$ Pictoris Moving Group ($\beta$PMG). We find that uncorrected gravitational redshift and convective blueshift bias absolute radial velocity measurements by $\sim$ 0.6 kms${}^{-1}$, which leads to erroneously younger traceback ages by $\sim$ 2 Myr. Random errors on parallax, proper motion, and radial velocity measurements lead to an additional bias of $\sim$ 1.5 Myr on traceback ages. Contamination of astrometric and kinematic data by kinematic outliers and unresolved multiple systems in the full input sample of 76 members and candidates of $\beta$PMG also erroneously lowers traceback ages by ${\sim}$ 3 Myr. We apply our new numerical traceback analysis tool to a core sample of 25 carefully vetted members of $\beta$PMG using Gaia Data Release 3 (DR3) data products and other kinematic surveys. Our method yields a corrected age of 20.4 $\pm$ 2.5 Myr, bridging the gap between kinematic ages (11$-$19 Myr) and other age-dating methods, such as isochrones and lithium depletion boundary (20$-$26 Myr). We explore several association size metrics that can track the spatial extent of $\beta$PMG over time, and we determine that minimizing the variance along the heliocentric curvilinear coordinate $\xi^{\prime}$ (i.e., toward the Galactic Center) offers the least random and systematic errors, due to the wider UVW space velocity dispersion of members of $\beta$PMG along the U-axis, which tends to maximize the spatial growth of the association along the $\xi^{\prime}$-axis over time.

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/age_distribution_beta_pictoris.tex <==
\begin{figure}
 	\includegraphics{age_distribution_beta_pictoris_fig.pdf}
    \caption{Traceback age distribution of \bpmg\ with 500 jackknife Monte Carlo iterations using a 50\,\% fraction, computed by minimizing the variance along the $\xi^\prime$-axis with a correction to account for the bias on traceback ages due to measurement errors (green). Our age estimate, \agecor, is compatible with other recent kinematic ages, i.e., \agemiretroigtrace\  (\citealp{2020AA...642A.179M}, orange) and \agecrundall\ (\citealp{2019MNRAS.489.3625C}, blue). However, all three age estimates remain incompatible with the range ages for \bpmg\  computed with the isochrones or LDB methods (\citealp{2014MNRAS.445.2169M}, light gray shaded area).}
 	\label{fig:beta_pictoris_4}
\end{figure}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/bias_error_age.tex <==
\begin{figure*}[!ht]
 	\includegraphics{bias_error_age_fig.pdf}
 	\caption{Bias (blue curves and circles) and error (green curves and squares) on the traceback age as a function of the initial $XYZ$ Galactic position scatter, the initial $UVW$ space velocity scatter, the radial velocity shift and measurement errors on radial velocity measurements, for $24$\,Myr old simulated NYAs made up of $25$ members each, using the $\xi^\prime$ variance as the association size metric. The bias on age is defined as the average measured age offset of simulated NYAs with respect to their actual age ($24$\,Myr), and the error on age is the standard deviation of the measured ages of simulated NYAs. Dotted and solid curves respectively represent the bias and error on the traceback age with and without the Galactic potential model I from \cite{2013AA...549A.137I}. The gray dashed line shows the actual simulated NYA's age. Simulation parameters are set to match members of the core sample of \bpmg: measurement errors on radial velocity, proper motion, and parallax are equal to average measurement errors of members of the core sample of \bpmg, the initial $XYZ$ Galactic position scatter is set to $3.0$\,pc, the initial $UVW$ space velocity scatter is set to $1.0$\,\kms, and the bias on radial velocity is set to $0.0$\,\kms. The results of simulations without the Galactic potential are similar to the results with the Galactic potential taken into account or only slightly offset, which seems to confirm our assumption that taking into account the effect of the Galactic potential has little impact on the final traceback age.}
 	\label{fig:simulated_samples}
\end{figure*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/convective_shift_spectral_type.tex <==
\begin{figure}
    \includegraphics{convective_shift_spectral_type_fig.pdf}
 	\caption{Convective blueshift (top panel) and total absolute radial velocity shift (bottom panel), including the effects of the gravitational redshift for main-sequence (solid purple line) and pre-main-sequence objects (dotted purple lines), as a function of spectral type. The shaded areas show the uncertainties based on individual spectral type measurement errors and propagated standard deviations of empirical mass and radius sequences. The convective blueshift three-segment polynomial sequence (solid blue line) was fitted with data from \cite{2017AA...607A.124M}, and the uncertainty was chosen to be wide enough to encompass data from: \cite{2019MNRAS.483.5026L}, \cite{2021AA...654A.168L}, \cite{2019ApJ...871..119D}, \cite{2020AA...641A..69B}, \cite{2019yCat..36240057L}, \cite{2013AA...550A.103A}, and \cite{1988AJ.....96..198G}, including measurements for YZ~CMi, a member of \bpmg, and the Sun.}
    \label{fig:conv_blueshift}
\end{figure}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/covariances_MAD_beta_pictoris.tex <==
\begin{figure}[t]
    \includegraphics{covariances_MAD_beta_pictoris_fig.pdf}
 	\caption{\bpmg\ size as a function of time, back to 35\,Myr into the past, using only members of the core sample. Several association size metrics are used: the determinant and trace of the empirical \xez\ covariance matrix, as well as the variance along the $\xi^\prime$-, $\eta^\prime$- and $\zeta^\prime$-axes (top panel), and the total \xez\ median absolute deviation (MAD) and the MAD along the same three axes (bottom panel). The epoch of minimal association size for each metric and its associated error are indicated in the legend.}
 	\label{fig:beta_pictoris_3}
\end{figure}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/error_ellipses_uvw.tex <==
\begin{figure*}
 	\includegraphics{error_ellipses_uvw_fig.pdf}
 	\caption{Application of the extreme deconvolution algorithm developed by \cite{2011AnApS...5.1657B} on the current-day $UVW$ space velocities of members of the core sample of \bpmg\ in order to mitigate the effect of the elongation of error bars along the line of sight due to relatively larger measurement errors on absolute radial velocity measurements. The dark and light blue shaded areas respectively represent the 67\,\% and 95\,\% probability ellipsoids defined by the diagonal terms of the covariance matrix. The length of the semi-major (a) and semi-minor (b) axes of the 95\,\% probability ellipsoids are indicated in the legends.}
 	\label{fig:error_ellipse_uvw}
\end{figure*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/gravitational_shift_spectral_type.tex <==
\begin{figure}[t]
    \includegraphics{gravitational_shift_spectral_type_fig.pdf}
 	\caption{Gravitational redshift as a function of spectral type based on our determinations of stellar masses and radii from empirical mass--spectral type and radius--spectral type sequences for main-sequence (solid red line) and pre-main-sequence objects (dotted red line). The shaded areas show the uncertainties based on individual spectral type measurement errors and propagated standard deviations of empirical mass and radius sequences. For most late-type members of \bpmg, the expected absolute radial velocity shifts due to the gravitational redshift alone are $\sim 0.6$\,\kms. For comparison, the radial velocity shifts due to the gravitational redshift of four stars within \bpmg\ that benefit from interferometric radius measurements are indicated by black circles and error bars \citep{2004IAUS..219...80K, 2008MNRAS.386.2039B, 2011ApJ...743..158S}.}
 	\label{fig:grav_redshift}
\end{figure}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/masses_radii_spectral_type.tex <==
\begin{figure*}[!ht]
    \includegraphics{masses_radii_spectral_type_with_zoom_fig.pdf}
 	\caption{Stellar masses (top panels) and radii (bottom panels) as a function of spectral type for field (blue circles) and young stars ($2-150$\,Myr, green triangles). The masses of both field and young stars were dynamically measured \citep{2004ApJ...604..741H, 2015ApJ...813L..11M, 2016AJ....152..175N, 2017AA...607A..10A, 2018AA...618A..23R,  2018AA...620A..33J, 2019ApJ...884...42S, 2021ApJ...908...46B, 2021ApJ...908...42P}. The radii of field stars were measured by interferometry \citep{2016AA...586A..94L} while the radii of young stars were derived from their SED using the modified P13 spectral type--radius relation \citep{2013ApJS..208....9P}, which reproduces empirical measurements at young ages, representative of \bpmg\ (magenta triangles). Blue ($> 200$\,Myr) and green ($\leq 200$\,Myr) lines represent our empirical spectral type--mass and spectral type--radius sequences with model extrapolations for spectral types later than M5 (light gray shaded area), for ages ranging from $1$\,Myr to $10$\,Gyr, using $50$ steps of $0.08$\,dex in log space. The discontinuity at $200$\,Myr is due to the adoption of distinct spectral type to effective temperature sequences as prescribed by \cite{2013ApJS..208....9P}. The error bars represent the typical uncertainty associated with our sequences for spectral types M5 and earlier (same colors), and the black error bar represents the uncertainty assigned to model extrapolations.}
 	\label{fig:masses_radii}
\end{figure*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_kinematics.tex <==
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 90}
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\begin{longrotatetable}
\begin{deluxetable*}{lcccccc}
\tablecolumns{7}
\tablecaption{The 6D kinematics of members of the core sample of \bpmg}
\label{tab:kinematics}
\tablehead{
    \colhead{Designation}    & \colhead{$X$} & \colhead{$Y$}          & \colhead{$Z$}         & \colhead{$U$}    & \colhead{$V$}  & \colhead{$W$}\\
    \colhead{}      & \colhead{(pc)}    & \colhead{(pc)} & \colhead{(pc)} & \colhead{(\kms)}                      & \colhead{(\kms)}      & \colhead{(\kms)}}
\startdata
RBS 38 & $14.64 \pm 0.01$ & $-18.64 \pm 0.02$ & $-28.27 \pm 0.01$ & $-10.9 \pm 0.2$ & $-15.6 \pm 0.3$ & $-7.9 \pm 0.3$\\
GJ 2006 A & $4.39 \pm 0.01$ & $-1.19 \pm 0.03$ & $-34.80 \pm 0.04$ & $-10.9 \pm 0.1$ & $-16.3 \pm 0.3$ & $-9.1 \pm 0.4$\\
HD 14082 B & $-27.93 \pm 0.02$ & $19.69 \pm 0.02$ & $-20.09 \pm 0.02$ & $-11.5 \pm 0.9$ & $-17 \pm 1$ & $-8 \pm 1$\\
AG Tri A & $-30.21 \pm 0.01$ & $20.29 \pm 0.01$ & $-18.98 \pm 0.02$ & $-12.6 \pm 0.2$ & $-15.5 \pm 0.2$ & $-8.3 \pm 0.2$\\
CD$-$57 1054 & $-1.544 \pm 0.006$ & $-21.332 \pm 0.006$ & $-16.337 \pm 0.004$ & $-11.1 \pm 0.5$ & $-16.1 \pm 0.6$ & $-8.8 \pm 0.4$\\
V1841 Ori & $-50.94 \pm 0.04$ & $-5.00 \pm 0.02$ & $-14.74 \pm 0.01$ & $-13.8 \pm 0.9$ & $-16.2 \pm 0.5$ & $-9.3 \pm 0.3$\\
BD$-$21 1074 A & $-12.390 \pm 0.006$ & $-11.349 \pm 0.004$ & $-10.571 \pm 0.002$ & $-12 \pm 1$ & $-15.3 \pm 0.8$ & $-7.9 \pm 0.5$\\
AO Men & $7.573 \pm 0.008$ & $-33.69 \pm 0.01$ & $-18.542 \pm 0.007$ & $-10.6 \pm 0.8$ & $-16 \pm 1$ & $-8.4 \pm 0.7$\\
UCAC2 12510535 & $30.35 \pm 0.01$ & $-10.07 \pm 0.01$ & $-1.240 \pm 0.008$ & $-9.7 \pm 0.4$ & $-16.2 \pm 0.3$ & $-10.2 \pm 0.2$\\
HD 164249 A & $45.51 \pm 0.04$ & $-15.11 \pm 0.04$ & $-11.95 \pm 0.02$ & $-8.0 \pm 0.3$ & $-16.2 \pm 0.3$ & $-9.1 \pm 0.2$\\
UCAC4 299$-$160704 & $55.11 \pm 0.05$ & $0.83 \pm 0.03$ & $-4.04 \pm 0.02$ & $-8.5 \pm 0.2$ & $-14.6 \pm 0.1$ & $-8.49 \pm 0.08$\\
2MASS J18092970$-$5430532 & $35.10 \pm 0.03$ & $-13.21 \pm 0.03$ & $-10.82 \pm 0.02$ & $-10.9 \pm 0.2$ & $-15.0 \pm 0.2$ & $-8.0 \pm 0.1$\\
1RXS J184206.5$-$555426 & $45.21 \pm 0.04$ & $-16.65 \pm 0.04$ & $-18.43 \pm 0.02$ & $-9.0 \pm 0.2$ & $-15.4 \pm 0.2$ & $-8.1 \pm 0.1$\\
Smethells 20 & $41.79 \pm 0.03$ & $-20.87 \pm 0.03$ & $-20.09 \pm 0.02$ & $-9.8 \pm 0.3$ & $-15.2 \pm 0.4$ & $-7.7 \pm 0.2$\\
CD$-$31 16041 & $48.05 \pm 0.03$ & $3.35 \pm 0.02$ & $-11.80 \pm 0.01$ & $-10 \pm 2$ & $-15 \pm 1$ & $-8.1 \pm 0.8$\\
HD 181327 & $41.04 \pm 0.04$ & $-12.72 \pm 0.04$ & $-21.18 \pm 0.03$ & $-9.2 \pm 0.2$ & $-15.3 \pm 0.2$ & $-7.8 \pm 0.1$\\
1RXS J192338.2$-$460631 & $64.45 \pm 0.06$ & $-9.16 \pm 0.06$ & $-29.69 \pm 0.04$ & $-7.6 \pm 0.2$ & $-16.4 \pm 0.2$ & $-9.5 \pm 0.1$\\
UCAC4 314$-$239934 & $57.79 \pm 0.06$ & $13.52 \pm 0.05$ & $-26.17 \pm 0.04$ & $-8.2 \pm 0.2$ & $-15.2 \pm 0.1$ & $-8.9 \pm 0.1$\\
TYC 7443$-$1102$-$1 & $45.36 \pm 0.03$ & $6.95 \pm 0.03$ & $-23.27 \pm 0.02$ & $-9.5 \pm 0.3$ & $-15.3 \pm 0.3$ & $-8.2 \pm 0.2$\\
UCAC4 284$-$205440 & $52.45 \pm 0.04$ & $7.27 \pm 0.04$ & $-28.53 \pm 0.03$ & $-8.0 \pm 0.5$ & $-15.9 \pm 0.4$ & $-9.0 \pm 0.3$\\
HD 191089 & $42.70 \pm 0.04$ & $12.26 \pm 0.03$ & $-23.45 \pm 0.03$ & $-9 \pm 1$ & $-15.4 \pm 0.7$ & $-9.0 \pm 0.7$\\
AU Mic & $7.593 \pm 0.001$ & $1.705 \pm 0.001$ & $-5.823 \pm 0.001$ & $-10.5 \pm 0.4$ & $-16.2 \pm 0.4$ & $-9.9 \pm 0.4$\\
GSC 06354$-$00357 & $22.00 \pm 0.02$ & $12.32 \pm 0.02$ & $-20.38 \pm 0.02$ & $-10.3 \pm 0.5$ & $-15.5 \pm 0.4$ & $-9.5 \pm 0.5$\\
CPD$-$72 2713 & $19.639 \pm 0.007$ & $-19.01 \pm 0.01$ & $-24.634 \pm 0.008$ & $-10.8 \pm 0.3$ & $-15.4 \pm 0.5$ & $-7.4 \pm 0.3$\\
WW PsA & $9.542 \pm 0.005$ & $2.117 \pm 0.008$ & $-18.46 \pm 0.01$ & $-10.7 \pm 0.2$ & $-16.2 \pm 0.3$ & $-9.8 \pm 0.3$\\
\enddata
\end{deluxetable*}
\end{longrotatetable}
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 0}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_multiple_systems.tex <==
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\startlongtable
\begin{deluxetable*}{lcccccc}
\tablecolumns{7}
\tablecaption{Multiplicity indicators of members of the input sample of \bpmg}
\label{tab:multiple}
\tablehead{
    \colhead{Designation}	& \colhead{Number}	& \colhead{RV}	& \colhead{\gaiadr}	& \colhead{CMD}	& \colhead{WDS} & \colhead{Literature}\\
    \colhead{}		& \colhead{of RVs$^{\textrm{a}}$}    	& \colhead{Variability$^{\textrm{b}}$}	    & \colhead{RUWE$^{\textrm{1}}$}		& \colhead{Bright}	    	& \colhead{Catalog$^{\textrm{2}}$}    &\colhead{}}
\startdata
\sidehead{\textbf{Core Sample}}
RBS 38 & 29 & No & 0.950 & No & No & No\\
GJ 2006 A & 35 & No & 1.806 & No & No & No\\
HD 14082 B & 16 & No & 1.008 & No & No & No\\
AG Tri A & 27 & No & 0.892 & No & No & No\\
CD$-$57 1054 & 61 & No & 1.005 & No & No & No\\
V1841 Ori & 18 & No & 1.025 & No & No & No\\
BD$-$21 1074 A & 30 & No & 1.278 & No & No & No\\
AO Men & 38 & No & 0.843 & No & No & No\\
UCAC2 12510535 & 20 & No & 0.952 & No & No & No\\
HD 164249 A & 70 & No & 1.093 & No & No & No\\
UCAC4 299$-$160704 & 7 & No & 0.655 & No & No & No\\
2MASS J18092970$-$5430532 & 22 & No & 1.440 & No & No & No\\
1RXS J184206.5$-$555426 & 33 & No & 1.262 & No & No & No\\
Smethells 20 & 27 & No & 1.029 & No & No & No\\
CD$-$31 16041 & 12 & No & 0.961 & No & \textbf{Yes} & \textbf{Yes}\\
HD 181327 & 94 & No & 0.961 & No & No & No\\
1RXS J192338.2$-$460631 & 25 & No & 1.276 & No & No & No\\
UCAC4 314$-$239934 & 14 & No & 1.267 & No & No & No\\
TYC 7443$-$1102$-$1 & 23 & No & 1.074 & No & \textbf{Yes} & No\\
UCAC4 284$-$205440 & 25 & No & 1.091 & No & No & No\\
HD 191089 & 56 & No & 0.878 & No & No & No\\
AU Mic & 100 & No & 0.927 & No & No & No\\
GSC 06354$-$00357 & 16 & No & 1.178 & No & No & No\\
CPD$-$72 2713 & 29 & No & 0.925 & No & No & No\\
WW PsA & 34 & No & 1.139 & No & No & No\\
\sidehead{\textbf{Extended Sample}}
HD 203 & 31 & \textbf{Yes} & 0.933 & No & No & No\\
LP 525$-$39 & 7 & \textbf{Slight} & 1.159 & No & No & \textbf{Yes}\\
GJ 3076 & 12 & \textbf{Slight} & ... & No & No & \textbf{Yes}\\
Barta 161 12 & 79 & \textbf{Slight} & 1.488 & No & No & \textbf{Yes}\\
PM J01538$-$1459A & 6 & No & 1.363 & No & No & \textbf{Yes}\\
EPIC 211046195 & \textbf{1} & ... & 1.217 & No & No & No\\
StKM 1$-$433 & 27 & \textbf{Slight} & 1.341 & No & No & No\\
51 Eri & 129 & \textbf{Slight} & 1.145 & No & No & No\\
2MASS J04433761$+$0002051 & \textbf{1} & ... & 1.140 & No & No & No\\
V1005 Ori & 65 & No & 0.900 & No & \textbf{Yes} & No\\
LP 476$-$207 & 34 & \textbf{Yes} & 1.254 & No & No & \textbf{Yes}\\
AF Lep & 78 & \textbf{Yes} & 0.918 & No & No & No\\
UCAC4 287$-$007048 & 28 & ... & 1.212 & No & No & No\\
V1311 Ori & 31 & No & \textbf{33.498} & No & \textbf{Yes} & \textbf{Yes}\\
$\beta$ Pic & 1507 & \textbf{Slight} & \textbf{3.072} & No & No & \textbf{Yes}\\
GSC 06513$-$00291 & 32 & No & \textbf{12.638} & No & \textbf{Yes} & \textbf{Yes}\\
TWA 22 A & 30 & No & \textbf{8.878} & No & No & \textbf{Yes}\\
$\alpha$ Cir & 4967 & \textbf{Slight} & \textbf{3.926} & No & No & No\\
V343 Nor A & 77 & \textbf{Slight} & \textbf{8.614} & No & No & \textbf{Yes}\\
UCAC3 89$-$246860 & 16 & ... & 1.448 & No & No & No\\
TYC 8726$-$1327$-$1 & 21 & No & \textbf{4.048} & No & No & \textbf{Yes}\\
2MASS J17020937$-$6734447 & 44 & ... & 1.286 & No & No & No\\
2MASS J17092947$-$5235197 & 10 & ... & \textbf{2.803} & No & No & No\\
HD 155555 A & 3 & \textbf{Yes} & 1.061 & No & \textbf{Yes} & No\\
CD$-$54 7336 & 21 & No & 0.897 & No & \textbf{Yes} & \textbf{Yes}\\
HD 160305 & 20 & \textbf{Slight} & 0.993 & No & No & No\\
UCAC4 184$-$193200 & 19 & ... & 1.211 & No & No & No\\
UCAC3 74$-$428746 & 15 & ... & 1.067 & No & No & No\\
UCAC3 66$-$407600 & 23 & \textbf{Slight} & 1.239 & No & No & No\\
HD 165189 & 16 & No & 1.137 & No & No & \textbf{Yes}\\
V4046 Sgr & 7 & \textbf{Yes} & 0.862 & No & \textbf{Yes} & \textbf{Yes}\\
UCAC3 63$-$445434 & 17 & ... & 1.368 & No & No & No\\
HD 168210 & 3 & ... & 0.728 & \textbf{Yes} & No & No\\
UCAC4 229$-$170667 & 16 & ... & 1.082 & No & No & No\\
UCAC4 226$-$179372 & 24 & ... & 1.010 & No & No & No\\
2MASS J18430597$-$4058047 & \textbf{1} & ... & 1.727 & No & No & No\\
HD 172555 & 571 & \textbf{Yes} & 1.069 & No & No & No\\
PZ Tel & 82 & \textbf{Yes} & 0.949 & No & No & \textbf{Yes}\\
TYC 6872$-$1011$-$1 & 11 & \textbf{Slight} & \textbf{2.372} & No & No & \textbf{Yes}\\
2MASS J19243494$-$3442392 & 17 & \textbf{Slight} & 1.497 & No & No & No\\
UCAC3 116$-$474938 & 11 & \textbf{Yes} & \textbf{29.710} & No & No & \textbf{Yes}\\
SCR J2010$-$2801 & 11 & \textbf{Slight} & \textbf{8.663} & No & No & \textbf{Yes}\\
SCR J2033$-$2556 & 6 & \textbf{Slight} & 1.961 & No & No & No\\
StHA 182 & 51 & \textbf{Slight} & 1.560 & No & No & \textbf{Yes}\\
HD 199143 & 5 & \textbf{Yes} & 1.033 & No & \textbf{Yes} & \textbf{Yes}\\
PSO J318.5338$-$22.8603 & \textbf{1} & ... & ... & No & No & No\\
TYC 9114$-$1267$-$1 & 62 & \textbf{Yes} & \textbf{48.126} & No & \textbf{Yes} & \textbf{Yes}\\
2E 4498 & 7 & \textbf{Yes} & \textbf{4.981} & No & No & No\\
HD 207043 & 41 & No & 0.863 & No & No & No\\
HD 213429 & 34 & \textbf{Yes} & ... & No & No & \textbf{Yes}\\
BD$-$13 6424 & 49 & \textbf{Slight} & 1.130 & No & No & No\\
\enddata
\tablecomments{RV: radial velocity; RUWE: Renormalized Unit Weight Error; CMD: color-magnitude diagram; WDS: Washington Double Star. Bold entries indicate a positive multiple system flag. (a)~See Table~\ref{tab:observations} for references for radial velocities. (b)~RV variability is present if the standard deviation of radial velocity measurements ($\sigma_{\textrm{RV}}$) is $> 2.0$\,\kms, slight if $0.6$\,\kms$\leq \sigma_{\textrm{RV}} \leq 2.0$\,\kms, and absent if $\sigma_{\textrm{RV}} < 0.6$\,\kms.}
\tablerefs{(1)~\citealp{2022arXiv220800211G}; (2)~\citealp{2022yCat....102026M}.}
\end{deluxetable*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_observations.tex <==
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 90}
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\begin{longrotatetable}
\begin{deluxetable*}{lllccccl}
\tablecolumns{8}
\tablecaption{Astrometric and kinematic measurements of members of the input  sample of \bpmg}
\label{tab:observations}
\tablehead{
    \colhead{Designation}    & \colhead{R.A.$^{\textrm{a}}$}          & \colhead{Decl.$^{\textrm{a}}$}         & \colhead{$\mu_\alpha \cos \delta$}    & \colhead{$\mu_\delta$}  & \colhead{$\pi$}  & \colhead{RV}  & \colhead{References$^{\textrm{b}}$}\\
    \colhead{}      & \colhead{(hh:mm:ss.ss)} & \colhead{(dd:mm:ss.ss)} & \colhead{(\masyr)}                      & \colhead{(\masyr)}      & \colhead{(mas)}    & \colhead{(\kms)}      & \colhead{}}
\startdata
\sidehead{\textbf{Core Sample}}
RBS 38 & 00:20:57.12 & $-$66:14:47.40 & $102.89 \pm 0.02$ & $-16.83 \pm 0.02$ & $27.16 \pm 0.02$ & $10.3 \pm 0.4$ & 1, 2, 3, 4, 5, 6\\
GJ 2006 A & 00:57:35.64 & $-$32:26:52.80 & $110.20 \pm 0.04$ & $-47.19 \pm 0.04$ & $28.55 \pm 0.04$ & $8.8 \pm 0.4$ & 1, 3, 5, 7\\
HD 14082 B & 02:21:20.88 & 28:44:40.92 & $86.86 \pm 0.03$ & $-74.17 \pm 0.03$ & $25.28 \pm 0.02$ & $4 \pm 2$ & 1, 8, 3, 9, 10, 11\\
AG Tri A & 02:52:20.28 & 30:58:23.52 & $79.54 \pm 0.02$ & $-72.13 \pm 0.01$ & $24.42 \pm 0.02$ & $6.0 \pm 0.3$ & 1, 8, 3, 12\\
CD$-$57 1054 & 05:11:48.12 & $-$57:44:35.88 & $35.39 \pm 0.01$ & $74.11 \pm 0.02$ & $37.21 \pm 0.01$ & $19.3 \pm 0.8$ & 1, 8, 2, 3, 13, 14, 15\\
V1841 Ori & 05:12:19.44 & 15:26:59.64 & $18.31 \pm 0.02$ & $-58.72 \pm 0.01$ & $18.83 \pm 0.02$ & $18 \pm 1$ & 1, 3, 16\\
BD$-$21 1074 A & 05:42:29.52 & $-$21:24:50.76 & $47.19 \pm 0.02$ & $-15.38 \pm 0.02$ & $50.43 \pm 0.02$ & $21 \pm 2$ & 1, 8, 2, 3, 10, 18\\
AO Men & 06:37:02.64 & $-$72:57:19.80 & $-7.71 \pm 0.02$ & $74.41 \pm 0.01$ & $25.57 \pm 0.01$ & $16 \pm 2$ & 1, 8, 2, 3, 13, 14, 9, 15\\
UCAC2 12510535 & 17:40:01.92 & $-$45:37:59.16 & $-20.10 \pm 0.02$ & $-137.84 \pm 0.02$ & $31.30 \pm 0.02$ & $-3.0 \pm 0.5$ & 1, 3\\
HD 164249 A & 18:45:51.12 & $-$51:21:02.16 & $2.33 \pm 0.02$ & $-86.23 \pm 0.02$ & $20.29 \pm 0.02$ & $0.2 \pm 0.4$ & 1, 8, 3, 13, 11, 15\\
UCAC4 299$-$160704 & 18:04:02.64 & $-$30:41:30.84 & $3.42 \pm 0.02$ & $-65.22 \pm 0.02$ & $18.15 \pm 0.02$ & $-7.4 \pm 0.1$ & 1, 3\\
2MASS J18092970$-$5430532 & 18:22:25.68 & $-$54:29:04.92 & $4.72 \pm 0.03$ & $-108.17 \pm 0.02$ & $25.67 \pm 0.03$ & $-1.9 \pm 0.3$ & 1, 3, 4\\
1RXS J184206.5$-$555426 & 18:31:44.76 & $-$55:05:33.00 & $12.01 \pm 0.02$ & $-79.07 \pm 0.01$ & $19.44 \pm 0.02$ & $0.6 \pm 0.2$ & 1, 3, 4, 5\\
Smethells 20 & 18:43:08.76 & $-$62:49:22.08 & $13.24 \pm 0.02$ & $-80.28 \pm 0.02$ & $19.72 \pm 0.02$ & $1.8 \pm 0.5$ & 1, 8, 2, 10, 15\\
CD$-$31 16041 & 18:41:07.44 & $-$31:12:11.52 & $17.27 \pm 0.02$ & $-72.34 \pm 0.01$ & $20.22 \pm 0.01$ & $-8 \pm 3$ & 1, 8, 19, 15\\
HD 181327 & 19:44:44.88 & $-$54:27:41.76 & $24.40 \pm 0.02$ & $-82.19 \pm 0.02$ & $20.93 \pm 0.03$ & $-0.1 \pm 0.2$ & 1, 8, 3, 13, 11, 15\\
1RXS J192338.2$-$460631 & 19:54:33.48 & $-$46:53:27.60 & $18.07 \pm 0.02$ & $-57.25 \pm 0.01$ & $14.03 \pm 0.02$ & $-0.2 \pm 0.2$ & 1, 3, 20, 5, 21, 6\\
UCAC4 314$-$239934 & 19:04:08.40 & $-$27:39:27.36 & $25.15 \pm 0.02$ & $-53.38 \pm 0.01$ & $15.47 \pm 0.02$ & $-6.26 \pm 0.05$ & 1, 3\\
TYC 7443$-$1102$-$1 & 19:01:06.24 & $-$32:52:21.36 & $33.60 \pm 0.02$ & $-68.53 \pm 0.01$ & $19.49 \pm 0.02$ & $-6.1 \pm 0.4$ & 1, 8, 2, 3, 5\\
UCAC4 284$-$205440 & 20:24:18.00 & $-$33:46:45.12 & $29.23 \pm 0.02$ & $-61.39 \pm 0.01$ & $16.68 \pm 0.02$ & $-4.0 \pm 0.6$ & 1, 8, 2, 3, 4, 10, 5\\
HD 191089 & 20:16:18.84 & $-$26:46:32.52 & $40.34 \pm 0.02$ & $-67.42 \pm 0.01$ & $19.96 \pm 0.02$ & $-7 \pm 1$ & 1, 8, 3, 13, 11, 16\\
AU Mic & 20:17:28.32 & $-$31:39:27.00 & $281.32 \pm 0.02$ & $-360.15 \pm 0.02$ & $102.94 \pm 0.02$ & $-4.5 \pm 0.6$ & 1, 8, 3, 13, 20, 11, 15\\
GSC 06354$-$00357 & 21:31:21.72 & $-$19:40:00.84 & $90.61 \pm 0.03$ & $-91.00 \pm 0.02$ & $30.90 \pm 0.03$ & $-6.2 \pm 0.8$ & 1, 2, 3, 4, 5, 21, 6\\
CPD$-$72 2713 & 22:42:18.72 & $-$71:17:38.04 & $94.85 \pm 0.01$ & $-52.38 \pm 0.01$ & $27.23 \pm 0.01$ & $7.8 \pm 0.6$ & 1, 8, 2, 3, 10, 15\\
WW PsA & 22:14:33.00 & $-$33:44:56.40 & $179.94 \pm 0.02$ & $-123.19 \pm 0.02$ & $47.92 \pm 0.03$ & $2.7 \pm 0.4$ & 1, 8, 3, 13, 5, 22, 15\\
\sidehead{\textbf{Extended Sample}}
HD 203 & 00:42:33.12 & $-$23:53:31.92 & $97.11 \pm 0.03$ & $-47.28 \pm 0.02$ & $25.16 \pm 0.03$ & $7 \pm 1$ & 1, 11, 15\\
LP 525$-$39 & 00:08:43.80 & 07:29:25.80 & $104.36 \pm 0.08$ & $-62.91 \pm 0.06$ & $28.43 \pm 0.06$ & $-3.7 \pm 0.6$ & 1, 3, 18\\
GJ 3076 & 01:51:24.48 & 15:26:20.04 & $187.6 \pm 0.8$ & $-120 \pm 1$ & $46 \pm 2$ & $2.5 \pm 0.3$ & 1, 23, 20, 5, 24, 18, 25\\
Barta 161 12 & 01:48:30.60 & $-$7:47:07.80 & $96.76 \pm 0.07$ & $-48.94 \pm 0.02$ & $26.82 \pm 0.05$ & $10 \pm 4$ & 1, 2, 26, 4, 27, 5, 7, 22\\
PM J01538$-$1459A & 01:27:44.64 & $-$14:00:08.64 & $106.72 \pm 0.04$ & $-40.60 \pm 0.03$ & $29.64 \pm 0.04$ & $9 \pm 4$ & 1, 2, 3, 5\\
EPIC 211046195 & 03:45:32.40 & 23:42:34.56 & $51.5 \pm 0.1$ & $-62.85 \pm 0.08$ & $19.72 \pm 0.09$ & $16 \pm 2$ & 1, 22\\
StKM 1$-$433 & 03:23:29.40 & 24:45:09.72 & $34.34 \pm 0.02$ & $-46.52 \pm 0.02$ & $14.55 \pm 0.02$ & $14 \pm 1$ & 1, 2, 3\\
51 Eri & 04:24:02.52 & $-$2:31:34.32 & $44.0 \pm 0.1$ & $-64.03 \pm 0.08$ & $33.44 \pm 0.08$ & $16 \pm 9$ & 1, 8, 13, 11\\
2MASS J04433761$+$0002051 & 04:54:24.84 & 00:02:03.48 & $55.3 \pm 0.2$ & $-107.3 \pm 0.2$ & $47.6 \pm 0.1$ & $17.0 \pm 0.8$ & 1, 28\\
V1005 Ori & 04:53:43.08 & 01:46:59.16 & $39.13 \pm 0.01$ & $-94.90 \pm 0.01$ & $40.99 \pm 0.01$ & $19.3 \pm 0.7$ & 1, 8, 3, 13, 12, 18\\
LP 476$-$207 & 05:29:42.36 & 09:58:57.00 & $31.66 \pm 0.04$ & $-121.57 \pm 0.02$ & $42.04 \pm 0.03$ & $18 \pm 6$ & 1, 3, 29, 11, 30, 18\\
AF Lep & 05:46:11.64 & $-$11:05:55.68 & $16.92 \pm 0.02$ & $-49.32 \pm 0.02$ & $37.25 \pm 0.02$ & $20.7 \pm 0.5$ & 1, 8, 31, 11, 16, 32, 33\\
UCAC4 287$-$007048 & 05:26:10.68 & $-$32:20:45.96 & $15.26 \pm 0.02$ & $10.77 \pm 0.02$ & $33.60 \pm 0.02$ & $22.0 \pm 0.8$ & 1, 20\\
V1311 Ori & 05:01:07.68 & $-$3:54:29.88 & $10.1 \pm 0.5$ & $-40.1 \pm 0.4$ & $29.0 \pm 0.6$ & $25 \pm 1$ & 1, 9, 3, 20, 34, 29, 10\\
$\beta$ Pic & 05:49:16.32 & $-$51:55:59.88 & $4.6 \pm 0.1$ & $83.1 \pm 0.2$ & $51.4 \pm 0.1$ & $12 \pm 7$ & 35, 1, 3, 13, 11\\
GSC 06513$-$00291 & 06:18:19.44 & $-$27:17:54.24 & $-14.2 \pm 0.2$ & $-1.2 \pm 0.2$ & $30.6 \pm 0.2$ & $25 \pm 6$ & 1, 9, 3, 20, 5\\
TWA 22 A & 10:21:38.88 & $-$53:05:33.36 & $-170.1 \pm 0.2$ & $-9.4 \pm 0.2$ & $50.5 \pm 0.2$ & $14.2 \pm 0.7$ & 1, 8, 3, 10, 36, 37\\
$\alpha$ Cir & 14:37:40.44 & $-$64:01:31.44 & $-192.5 \pm 0.1$ & $-233.5 \pm 0.1$ & $60.4 \pm 0.1$ & $7.1 \pm 0.2$ & 35, 3, 13, 14, 38, 11\\
V343 Nor A & 15:44:21.84 & $-$57:17:31.20 & $-49.86 \pm 0.06$ & $-97.87 \pm 0.07$ & $24.99 \pm 0.06$ & $3 \pm 2$ & 1, 9, 8, 3, 13, 11, 15\\
UCAC3 89$-$246860 & 16:01:16.68 & $-$45:03:34.20 & $-33.49 \pm 0.03$ & $-104.29 \pm 0.02$ & $22.91 \pm 0.03$ & $30 \pm 10$ & 1, 3\\
TYC 8726$-$1327$-$1 & 16:20:03.48 & $-$53:16:27.12 & $-12.9 \pm 0.1$ & $-85.26 \pm 0.08$ & $19.69 \pm 0.09$ & $1.4 \pm 0.1$ & 1, 3, 20, 5\\
2MASS J17020937$-$6734447 & 17:32:19.68 & $-$67:25:13.80 & $-20.36 \pm 0.02$ & $-99.53 \pm 0.02$ & $24.19 \pm 0.02$ & $5.7 \pm 0.3$ & 1, 3\\
2MASS J17092947$-$5235197 & 17:22:21.72 & $-$52:24:39.24 & $-8.83 \pm 0.06$ & $-67.94 \pm 0.05$ & $15.66 \pm 0.05$ & $1 \pm 6$ & 1, 3\\
HD 155555 A & 17:21:21.60 & $-$66:02:54.24 & $-21.44 \pm 0.01$ & $-137.17 \pm 0.01$ & $32.95 \pm 0.02$ & $-20 \pm 30$ & 1, 3, 11, 15\\
CD$-$54 7336 & 17:28:45.84 & $-$54:44:10.32 & $-5.49 \pm 0.01$ & $-63.44 \pm 0.01$ & $14.79 \pm 0.01$ & $1 \pm 1$ & 1, 8, 38, 10, 19, 15\\
HD 160305 & 17:27:15.48 & $-$50:16:31.08 & $-2.06 \pm 0.02$ & $-65.95 \pm 0.02$ & $15.20 \pm 0.02$ & $1.3 \pm 0.5$ & 1, 19\\
UCAC4 184$-$193200 & 17:10:38.64 & $-$53:44:11.40 & $-1.25 \pm 0.02$ & $-82.98 \pm 0.02$ & $18.81 \pm 0.02$ & $1.6 \pm 0.2$ & 1, 3\\
UCAC3 74$-$428746 & 17:08:26.16 & $-$53:53:47.40 & $-1.71 \pm 0.02$ & $-55.96 \pm 0.01$ & $13.05 \pm 0.02$ & $1.3 \pm 0.7$ & 1, 3\\
UCAC3 66$-$407600 & 18:28:44.04 & $-$57:55:28.20 & $0.89 \pm 0.02$ & $-72.95 \pm 0.02$ & $17.71 \pm 0.02$ & $-0.1 \pm 0.4$ & 1, 3, 4\\
HD 165189 & 18:42:28.80 & $-$43:34:27.48 & $10.9 \pm 0.1$ & $-105.84 \pm 0.08$ & $22.7 \pm 0.1$ & $-6 \pm 4$ & 1, 11\\
V4046 Sgr & 18:32:37.32 & $-$32:12:24.48 & $3.51 \pm 0.02$ & $-52.72 \pm 0.02$ & $13.99 \pm 0.02$ & $-20 \pm 20$ & 1, 3, 20, 10, 5\\
UCAC3 63$-$445434 & 18:03:06.12 & $-$58:15:52.20 & $14.14 \pm 0.02$ & $-146.54 \pm 0.02$ & $32.98 \pm 0.03$ & $3.2 \pm 0.4$ & 1, 3\\
HD 168210 & 18:58:03.36 & $-$29:43:26.40 & $4.58 \pm 0.02$ & $-46.41 \pm 0.02$ & $12.43 \pm 0.02$ & $-7 \pm 3$ & 1, 15\\
UCAC4 229$-$170667 & 18:04:07.68 & $-$44:38:11.40 & $5.01 \pm 0.02$ & $-51.28 \pm 0.02$ & $12.42 \pm 0.02$ & $-1.6 \pm 0.4$ & 1, 3\\
UCAC4 226$-$179372 & 18:08:48.84 & $-$44:02:31.20 & $4.81 \pm 0.02$ & $-49.52 \pm 0.01$ & $11.96 \pm 0.01$ & $-1.5 \pm 0.6$ & 1, 3\\
2MASS J18430597$-$4058047 & 18:46:30.00 & $-$40:01:54.12 & $12.08 \pm 0.04$ & $-71.22 \pm 0.03$ & $17.10 \pm 0.03$ & $3.9 \pm 0.2$ & 1, 3\\
HD 172555 & 18:21:44.64 & $-$64:07:41.16 & $31.95 \pm 0.09$ & $-149.7 \pm 0.1$ & $34.7 \pm 0.2$ & $-10 \pm 10$ & 1, 3, 13, 11, 15\\
PZ Tel & 18:16:28.56 & $-$50:49:08.76 & $16.27 \pm 0.02$ & $-85.52 \pm 0.02$ & $21.16 \pm 0.02$ & $-20 \pm 80$ & 1, 8, 3, 13, 11, 15\\
TYC 6872$-$1011$-$1 & 18:31:02.64 & $-$29:06:54.72 & $13.63 \pm 0.05$ & $-48.15 \pm 0.04$ & $13.45 \pm 0.04$ & $-6 \pm 2$ & 1, 8, 21, 15\\
2MASS J19243494$-$3442392 & 19:08:44.88 & $-$34:17:19.32 & $26.37 \pm 0.03$ & $-75.60 \pm 0.03$ & $19.40 \pm 0.03$ & $-4 \pm 1$ & 1, 3, 4, 5\\
UCAC3 116$-$474938 & 19:00:44.64 & $-$32:52:40.08 & $33.1 \pm 0.7$ & $-73.0 \pm 0.5$ & $19.5 \pm 0.7$ & $-10 \pm 20$ & 1, 8, 2, 3, 4, 10, 5\\
SCR J2010$-$2801 & 20:30:01.80 & $-$28:58:17.76 & $47.6 \pm 0.3$ & $-74.5 \pm 0.2$ & $21.6 \pm 0.3$ & $-7 \pm 5$ & 1, 3, 4, 5\\
\enddata
\tablecomments{(a)~All right ascensions (R.A.) and declinations (decl.) are sourced from \gaiadr\ \citep{2022arXiv220800211G}.  All positions are given at the $2016$ epoch, except for PSO J318.5338$-$22.8603, for which the epoch is $2011.563872$. (b)~References are given for proper motions ($\mu_\alpha \cos \delta$ and $\mu_\delta$), parallaxes ($\pi$) and radial velocities (RV) respectively.}
\tablerefs{(1)~\citealp{2022arXiv220800211G}; (2)~\citealp{2020AJ....160..120J}; (3)~\citealp{2020AA...642A.179M}; (4)~\citealp{2017AJ....154...69S}; (5)~\citealp{2014ApJ...788...81M}; (6)~\citealp{2013ApJ...762...88M}; (7)~\citealp{2014AJ....147..146K}; (8)~\citealp{2021AA...645A..30Z}; (9)~\citealp{2016AA...596A.116S}; (10)~\citealp{2020AA...636A..74T}; (11)~\citealp{2018AA...616A...7S}; (12)~\citealp{2006AA...460..695T}; (13)~\citealp{2007AJ....133.2524W}; (14)~\citealp{ 2007AJ....133.2524W}; (15)~\citealp{2014AA...568A..26E}; (16)~\citealp{2002AJ....123.3356G}; (17)~\citealp{2018AA...616A...1G}; (18)~\citealp{2007AN....328..889K}; (19)~\citealp{2012AJ....144....8S}; (20)~\citealp{2019AJ....157..234S}; (21)~\citealp{2013MNRAS.435.1376M}; (22)~\citealp{2012ApJ...758...56S}; (23)~\citealp{2014AJ....147...85R}; (24)~\citealp{2014AJ....147...20N}; (25)~\citealp{2001MNRAS.328...45M}; (26)~\citealp{2020AA...636A..36L}; (27)~\citealp{2014MNRAS.438L..11B}; (28)~\citealp{2016ApJS..225...10F}; (29)~\citealp{2016MNRAS.455.3345B}; (30)~\citealp{2003ApJ...599..342S}; (31)~\citealp{2013ApJS..209...33M}; (32)~\citealp{2005ApJS..159..141V}; (33)~\citealp{2001AA...379..976M}; (34)~\citealp{2018AA...618A...5D}; (35)~\citealp{2007AA...474..653V}; (36)~\citealp{2011ApJ...727....6S}; (37)~\citealp{2009AA...503..281T}; (38)~\citealp{2015AA...573A.126D}; (39)~\citealp{2004AA...418..989N}; (40)~\citealp{2016ApJ...833...96L}; (41)~\citealp{2016ApJ...819..133A}; (42)~\citealp{2018AA...614A..76J}; (43)~\citealp{2013AJ....145...41K}.}
\end{deluxetable*}
\end{longrotatetable}
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 0}
%\tablenotetext{a}{All parallaxes and proper motions are from Gaia~EDR3.}



==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_parameters.tex <==
\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\begin{deluxetable}{lc}[t]
\tablecolumns{2}
\tablecaption{Parameters of the input and core samples of \bpmg}
\label{tab:parameters}
\tablehead{\colhead{Parameter} & \colhead{Value}}
\startdata
\sidehead{\textbf{Input Sample}}
Number of stars & 76\\
Average distance & $28.22 \pm 0.02$\,pc\\
Distance range & $9.719-83.99$\,pc\\
$XYZ$ & ($22.14$, $-5.20$, $-16.71$)\,pc\\
$\sigma_{XYZ}$ & ($32.97$, $14.08$, $8.61$)\,pc\\
$UVW$ & ($-10$, $-15$, $-9$)\,\kms\\
$\sigma_{UVW}$ & ($8$, $5$, $5$)\,\kms\\
\sidehead{\textbf{Core Sample}}
Number of stars & 25\\
Average distance & $29.587 \pm 0.006$\,pc\\
Distance range & $9.719-71.55$\,pc\\
$XYZ$ & ($22.691$, $-4.308$, $-18.492$)\,pc\\
$\sigma_{XYZ}$ & ($29.698$, $13.940$, $8.106$)\,pc\\
$UVW$ & ($-10.2$, $-15.7$, $-8.64$)\,\kms\\
$\sigma_{UVW}$ & ($1.5$, $0.6$, $0.76$)\,\kms\\
\enddata
\tablecomments{The average $XYZ$ Galactic position and dispersion ($\sigma_{XYZ}$) and the average $UVW$ space velocity and dispersion ($\sigma_{UVW}$) are given for members of the input and core samples of \bpmg.}
\end{deluxetable}

%\begin{align}\label{eq:average_xyz_uvw}
%X &= 18.7\textrm{\,pc} & U &= -10.3\textrm{\,\kms}\notag\\
%Y &= -4.5\textrm{\,pc} & V &= -15.7\textrm{\,\kms}\\
%Z &= -18.9\textrm{\,pc} & W &= -8.8\textrm{\,\kms}\notag
%\end{align}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_rv_shift.tex <==
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\begin{longrotatetable}
\begin{deluxetable*}{llccccccl}
\tablecolumns{9}
\tablecaption{Gravitational redshift and convective blueshift on radial velocity measurements of members of the core sample of \bpmg}
\label{tab:rv_shift}
\tablehead{
    \colhead{Designation} &
    \colhead{Spectral} & 
    \colhead{Mass$^{\textrm{b}}$} &
    \colhead{Radius$^{\textrm{b}}$} &
    \colhead{$\Delta$RV${}_{\textrm{grav.}}$} &
    \colhead{$\Delta$RV${}_{\textrm{conv.}}$} &
    \colhead{$\Delta$RV${}_{\textrm{total}}$} &
    \colhead{RV${}_{\textrm{cor.}}$} &
    \colhead{References$^{\textrm{c}}$}\\
    \colhead{} &
    \colhead{Type$^{\textrm{a}}$} &
    \colhead{(\msol)} &
    \colhead{(\rsol)}&
    \colhead{(\kms)} &
    \colhead{(\kms)} &
    \colhead{(\kms)} &
    \colhead{(\kms)} &
    \colhead{}}
\startdata
RBS 38 & M2.5V & $0.40 \pm 0.04$ & $0.39 \pm 0.04$ & $0.66 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $9.6 \pm 0.6$ & 1, 2\\
GJ 2006 A & M3.5Ve & $0.26 \pm 0.03$ & $0.31 \pm 0.03$ & $0.61 \pm 0.08$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $8.2 \pm 0.6$ & 1, 2\\
HD 14082 B & G2V & $1.0 \pm 0.1$ & $1.1 \pm 0.1$ & $0.62 \pm 0.09$ & $-0.4 \pm 0.2$ & $0.3 \pm 0.2$ & $4 \pm 2$ & 1, 2\\
AG Tri A & K8V & $0.59 \pm 0.06$ & $0.60 \pm 0.05$ & $0.64 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $5.4 \pm 0.5$ & 1, 2\\
CD$-$57 1054 & K8Ve & $0.59 \pm 0.06$ & $0.60 \pm 0.05$ & $0.64 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $18.7 \pm 0.9$ & 1, 2\\
V1841 Ori & K2IV & $0.78 \pm 0.08$ & $0.77 \pm 0.07$ & $0.66 \pm 0.09$ & $-0.1 \pm 0.2$ & $0.5 \pm 0.2$ & $17 \pm 1$ & 1, 2\\
BD$-$21 1074 A & M1V & $0.49 \pm 0.05$ & $0.50 \pm 0.04$ & $0.65 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $21 \pm 2$ & 1, 2\\
AO Men & K3.5V & $0.73 \pm 0.08$ & $0.73 \pm 0.07$ & $0.65 \pm 0.09$ & $-0.1 \pm 0.2$ & $0.6 \pm 0.2$ & $16 \pm 2$ & 1, 2\\
UCAC2 12510535 & (M2) & $0.44 \pm 0.05$ & $0.43 \pm 0.04$ & $0.66 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-3.7 \pm 0.7$ & 1, 2\\
HD 164249 A & F4.5V & $1.4 \pm 0.2$ & $1.5 \pm 0.1$ & $0.59 \pm 0.08$ & $-0.2 \pm 0.2$ & $0.4 \pm 0.2$ & $-0.2 \pm 0.6$ & 1, 2\\
UCAC4 299$-$160704 & (M2) & $0.44 \pm 0.05$ & $0.43 \pm 0.04$ & $0.66 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-8.0 \pm 0.5$ & 1, 2\\
2MASS J18092970$-$5430532 & (M4) & $0.22 \pm 0.02$ & $0.27 \pm 0.02$ & $0.58 \pm 0.08$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-2.5 \pm 0.6$ & 1, 2\\
1RXS J184206.5$-$555426 & M3.5V & $0.26 \pm 0.03$ & $0.31 \pm 0.03$ & $0.61 \pm 0.08$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-0.0 \pm 0.5$ & 1, 2\\
Smethells 20 & M1Ve & $0.49 \pm 0.05$ & $0.50 \pm 0.04$ & $0.65 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $1.2 \pm 0.7$ & 1, 2\\
CD$-$31 16041 & K8IVe & $0.59 \pm 0.06$ & $0.60 \pm 0.05$ & $0.64 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-9 \pm 3$ & 1, 2\\
HD 181327 & F6V & $1.2 \pm 0.1$ & $1.4 \pm 0.1$ & $0.59 \pm 0.08$ & $-0.3 \pm 0.2$ & $0.2 \pm 0.2$ & $-0.3 \pm 0.5$ & 1, 2\\
1RXS J192338.2$-$460631 & M0V & $0.55 \pm 0.06$ & $0.55 \pm 0.05$ & $0.65 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-0.8 \pm 0.5$ & 1, 2\\
UCAC4 314$-$239934 & (M2) & $0.44 \pm 0.05$ & $0.43 \pm 0.04$ & $0.66 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-6.9 \pm 0.5$ & 1, 2\\
TYC 7443$-$1102$-$1 & K9IVe & $0.56 \pm 0.06$ & $0.57 \pm 0.05$ & $0.64 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-6.7 \pm 0.6$ & 1, 2\\
UCAC4 284$-$205440 & M1V & $0.49 \pm 0.05$ & $0.50 \pm 0.04$ & $0.65 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-4.6 \pm 0.8$ & 1, 2\\
HD 191089 & F5V & $1.3 \pm 0.1$ & $1.4 \pm 0.1$ & $0.59 \pm 0.08$ & $-0.3 \pm 0.2$ & $0.3 \pm 0.2$ & $-8 \pm 1$ & 1, 2\\
AU Mic & M0Ve & $0.55 \pm 0.06$ & $0.55 \pm 0.05$ & $0.65 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-5.2 \pm 0.8$ & 1, 2\\
GSC 06354$-$00357 & M2V & $0.44 \pm 0.05$ & $0.43 \pm 0.04$ & $0.66 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $-6.9 \pm 0.9$ & 1, 2\\
CPD$-$72 2713 & K7IVe & $0.63 \pm 0.07$ & $0.62 \pm 0.06$ & $0.64 \pm 0.09$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $7.2 \pm 0.8$ & 1, 2\\
WW PsA & M4IVe & $0.22 \pm 0.02$ & $0.27 \pm 0.02$ & $0.58 \pm 0.08$ & $-0.0 \pm 0.2$ & $0.6 \pm 0.2$ & $2.2 \pm 0.6$ & 1, 2\\
\enddata
\tablecomments{$\Delta$RV${}_{\textrm{grav.}}$: gravitational radial velocity shift;$\Delta$RV${}_{\textrm{conv.}}$ convective radial velocity shift; $\Delta$RV${}_{\textrm{total}}$: total radial velocity shift; RV${}_{\textrm{cor.}}$: corrected radial velocity. (a)~Parentheses indicate that the spectral type was inferred from a photometric estimate based on the \gaiagr\ color. See Table~\ref{tab:sample} for references for spectral types. (b)~See Figure~\ref{fig:masses_radii} for details on stellar masses and radii determination. (c)~References are given for stellar mass and radius, respectively.}
\tablerefs{(1)~This paper; (2)~\citealp{2013ApJS..208....9P}.}
\end{deluxetable*}
\end{longrotatetable}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_sample.tex <==
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\startlongtable
\begin{deluxetable*}{lllll}
\tablecolumns{5}
\tablecaption{Members of the input sample of \bpmg}
\label{tab:sample}
\tablehead{
    \colhead{Designation}	& \colhead{\gaiadr\ ID} & \colhead{2MASS ID}& \colhead{Spectral}            & \colhead{References$^{\textrm{b}}$}\\
    \colhead{}              & \colhead{}            & \colhead{}        & \colhead{type$^{\textrm{a}}$}	& \colhead{}}
\startdata
\sidehead{\textbf{Core Sample}}
RBS 38 & 4707563810327288192 & J00172353$-$6645124 & M2.5V & 1, 2, 3\\
GJ 2006 A & 2315841869173294080 & J00275023$-$3233060 & M3.5Ve & 2, 3\\
HD 14082 B & 107774198474602368 & J02172472$+$2844305 & G2V & 4, 5, 6\\
AG Tri A & 132362959259196032 & J02272924$+$3058246 & K8V & 4, 7, 6\\
CD$-$57 1054 & 4764027962957023104 & J05004714$-$5715255 & K8Ve & 8, 5, 9\\
V1841 Ori & 3393207610483520896 & J05004928$+$1527006 & K2IV & 10, 11\\
BD$-$21 1074 A & 2962658549474035584 & J05064991$-$2135091 & M1V & 12, 1\\
AO Men & 5266270443442455040 & J06182824$-$7202416 & K3.5V & 8, 5, 9\\
UCAC2 12510535 & 5963633872326630272 & J17024014$-$4521587 & (M2) & 13\\
HD 164249 A & 6702775135228913280 & J18030341$-$5138564 & F4.5V & 9, 5\\
UCAC4 299$-$160704 & 4050178830427649024 & J18041617$-$3018280 & (M2) & 13\\
2MASS J18092970$-$5430532 & 6653162456161626368 & J18092970$-$5430532 & (M4) & 14, 13\\
1RXS J184206.5$-$555426 & 6649788119394186112 & J18420694$-$5554254 & M3.5V & 1, 3\\
Smethells 20 & 6631685008336771072 & J18465255$-$6210366 & M1Ve & 15, 5, 9\\
CD$-$31 16041 & 6736232346363422336 & J18504448$-$3147472 & K8IVe & 15, 9\\
HD 181327 & 6643589352010758400 & J19225894$-$5432170 & F6V & 8, 5, 9\\
1RXS J192338.2$-$460631 & 6663346029775435264 & J19233820$-$4606316 & M0V & 1, 2, 16\\
UCAC4 314$-$239934 & 6754492966739292928 & J19481651$-$2720319 & (M2) & 13\\
TYC 7443$-$1102$-$1 & 6747467224874108288 & J19560438$-$3207376 & K9IVe & 1, 5, 2\\
UCAC4 284$-$205440 & 6747106443324127488 & J20013718$-$3313139 & M1V & 1, 2\\
HD 191089 & 6847146784384459648 & J20090521$-$2613265 & F5V & 1, 11\\
AU Mic & 6794047652729201024 & J20450949$-$3120266 & M0Ve & 8, 5, 16\\
GSC 06354$-$00357 & 6833292181958100224 & J21100535$-$1919573 & M2V & 1, 2\\
CPD$-$72 2713 & 6382640367603744128 & J22424896$-$7142211 & K7IVe & 15, 5, 9\\
WW PsA & 6603693881832177792 & J22445794$-$3315015 & M4IVe & 4, 9\\
\sidehead{\textbf{Extended Sample}}
HD 203 & 2337191189529102336 & J00065008$-$2306271 & F3V & 8, 5, 9\\
LP 525$-$39 & 2749470902772705408 & J00323480$+$0729271 & M3Ve & 17, 18\\
GJ 3076 & 2783378162041480832 & J01112542$+$1526214 & M5 & 1, 16\\
Barta 161 12 & 2477870708709917568 & J01351393$-$0712517 & M4.3 & 19, 3\\
PM J01538$-$1459A & 5143033331902438656 & J01535076$-$1459503 & M3V & 1, 2\\
EPIC 211046195 & 68012529415816832 & J03350208$+$2342356 & M8.5 & 19\\
StKM 1$-$433 & 66245408072670336 & J03573393$+$2445106 & M2 & 13, 20\\
51 Eri & 3205095125321700480 & J04373613$-$0228248 & F0IV & 8, 21\\
2MASS J04433761$+$0002051 & 3230008650057256960 & J04433761$+$0002051 & M9$\gamma$ & 22, 23\\
V1005 Ori & 3231945508509506176 & J04593483$+$0147007 & K8IVe & 15, 5, 9\\
LP 476$-$207 & 3291643148740384128 & J05015881$+$0958587 & M4IVe & 4, 5, 6\\
AF Lep & 3009908378049913216 & J05270477$-$1154033 & F7V & 8, 5, 11\\
UCAC4 287$-$007048 & 2901786974419551488 & J05294468$-$3239141 & M4.5 & 16, 9\\
V1311 Ori & 3216729573251961856 & J05320450$-$0305291 & M2Ve & 1, 16\\
$\beta$ Pic & 4792774797545800832 & J05471708$-$5103594 & A6V & 8, 24\\
GSC 06513$-$00291 & 2899492637251200512 & J06131330$-$2742054 & M3.5V & 1, 2, 16\\
TWA 22 A & 5355751581627180288 & J10172689$-$5354265 & M5 & 4, 25\\
$\alpha$ Cir & 5849837854861497856 & J14423039$-$6458305 & A7V & 13, 24\\
V343 Nor A & 5882581895219921024 & J15385757$-$5742273 & G8V & 8, 5, 9\\
UCAC3 89$-$246860 & 5990286858802698752 & J16120516$-$4556242 & (M4) & 13\\
TYC 8726$-$1327$-$1 & 5935776714456619008 & J16572029$-$5343316 & M3V & 1, 2, 16\\
2MASS J17020937$-$6734447 & 5814416056916139520 & J17020937$-$6734447 & (M4) & 13\\
2MASS J17092947$-$5235197 & 5924347802133154944 & J17092947$-$5235197 & (M3) & 13\\
HD 155555 A & 5811866422581688320 & J17172550$-$6657039 & G5V & 8, 5\\
CD$-$54 7336 & 5924485966955008896 & J17295506$-$5415487 & K1V & 9\\
HD 160305 & 5946515438335508864 & J17414903$-$5043279 & F9V & 26\\
UCAC4 184$-$193200 & 5921821644117633152 & J17444256$-$5315471 & (M3) & 13\\
UCAC3 74$-$428746 & 5945104588806333824 & J17483374$-$5306118 & (M2) & 13\\
UCAC3 66$-$407600 & 6648834361774839040 & J18055491$-$5704307 & (M2) & 14, 13\\
HD 165189 & 6724105656508792576 & J18064990$-$4325297 & A6V & 8, 27\\
V4046 Sgr & 4045698423617983488 & J18141047$-$3247344 & K4IVe & 15, 5, 16\\
UCAC3 63$-$445434 & 6647518766053564544 & J18161236$-$5844055 & M3.5Ve & 13, 28\\
HD 168210 & 4051081838710783232 & J18195221$-$2916327 & G3IV & 15, 5, 9\\
UCAC4 229$-$170667 & 6721666531703090432 & J18281651$-$4421477 & (M2) & 13\\
UCAC4 226$-$179372 & 6709580695582315648 & J18283524$-$4457280 & (K7) & 13\\
2MASS J18430597$-$4058047 & 6728469996119674112 & J18430597$-$4058047 & (M2) & 13\\
HD 172555 & 6438274350302427776 & J18452691$-$6452165 & A7 & 8\\
PZ Tel & 6655168686921108864 & J18530587$-$5010499 & G9IV & 8, 9\\
TYC 6872$-$1011$-$1 & 6760846563417053056 & J18580415$-$2953045 & K8IVe & 15, 5, 9\\
2MASS J19243494$-$3442392 & 6742986538895222144 & J19243494$-$3442392 & M4V & 1, 2, 3\\
UCAC3 116$-$474938 & 6747467431032539008 & J19560294$-$3207186 & M4V & 1, 2\\
SCR J2010$-$2801 & 6846651450099142016 & J20100002$-$2801410 & M2.5 & 1, 3\\
SCR J2033$-$2556 & 6800238044930953600 & J20333759$-$2556521 & M4.5V & 1, 2\\
StHA 182 & 6806301370521783552 & J20434114$-$2433534 & M3.7 & 1, 2\\
HD 199143 & 6882840883188886784 & J20554767$-$1706509 & F7V & 8, 29, 9\\
PSO J318.5338$-$22.8603 & ... & J21140802$-$2251358 & L7 & 22, 30\\
TYC 9114$-$1267$-$1 & 6400160947954197888 & J21212873$-$6655063 & K7V & 31, 2, 16\\
2E 4498 & 2694353690543010560 & J21374019$+$0137137 & M5 & 10, 14\\
HD 207043 & 6462296480342791808 & J21475527$-$5255502 & G5V & 32, 24\\
HD 213429 & 2622845684814477696 & J22311828$-$0633183 & F8V & 13, 33\\
BD$-$13 6424 & 2433191886212246784 & J23323085$-$1215513 & M0V$-$IVe & 15, 5, 9\\
\enddata
\tablecomments{(a)~Parentheses indicate that the spectral type was inferred from a photometric estimate based on the \gaiagr\ color. (b)~References are given for membership and spectral types respectively.}
\tablerefs{(1)~\citealp{2013ApJ...762...88M}; (2)~\citealp{2014ApJ...788...81M}; (3)~\citealp{2017ApJ...840...87R}; (4)~\citealp{2003ApJ...599..342S}; (5)~\citealp{1987AJ.....93..959R}; (6)~\citealp{1992AA...258..217E}; (7)~\citealp{2001ApJ...562L..87Z}; (8)~\citealp{2013ApJS..208....9P}; (9)~\citealp{2006AA...460..695T}; (10)~\citealp{2012AJ....143...80S}; (11)~\citealp{2007AJ....133.2524W}; (12)~\citealp{2009AA...508..833D}; (13)~\citealp{2018ApJ...862..138G}; (14)~\citealp{2017AJ....154...69S}; (15)~\citealp{2010AA...520A..15M}; (16)~\citealp{2019AJ....157..234S}; (17)~\citealp{2012AJ....144..109S}; (18)~\citealp{1986AJ.....92..139S}; (19)~\citealp{2012ApJ...758...56S}; (20)~\citealp{2012AJ....143..114S}; (21)~\citealp{1988mcts.book.....H}; (22)~\citealp{2014ApJ...783..121G}; (23)~\citealp{2013ApJ...772...79A}; (24)~\citealp{2006AJ....132..161G}; (25)~\citealp{1993AJ....105.1962W}; (26)~\citealp{2011MNRAS.411..117K}; (27)~\citealp{1984ApJS...55..657C}; (28)~\citealp{2018AJ....156...49R}; (29)~\citealp{1978mcts.book.....H}; (30)~\citealp{2013ApJ...777L..20L}; (31)~\citealp{2010AJ....140..119S}; (32)~\citealp{2018ApJ...860...43G}; (33)~\citealp{2003AJ....126.2048G}.}
\end{deluxetable*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/table_size_metrics.tex <==
%\tablewidth{\textwidth}
%\tabletypesize{\normalsize}
%\tabletypesize{\footnotesize}
\tabletypesize{\small}
\startlongtable
\begin{deluxetable*}{lccccc}
\tablecolumns{6}
\tablecaption{Traceback Ages of \bpmg}
\label{tab:size_metrics}
\tablehead{
    \colhead{Association Size Metric}	& \colhead{Age}	    & \colhead{Jackknife Error$^{\textrm{a}}$}	& \colhead{Measurement Error$^{\textrm{a}}$}	& \colhead{Total Error$^{\textrm{a}}$}	& \colhead{Contrast$^{\textrm{b}}$}\\
    \colhead{}			    & \colhead{(Myr)}	& \colhead{(Myr)}			    & \colhead{(Myr)}				& \colhead{(Myr)}		& \colhead{(\%)}}
\startdata
\sidehead{\textbf{Spatial Covariance Matrix}}
\bm{$X$} \textbf{Variance} & \bm{$19.0$} & \bm{$2.3$} & \bm{$1.6$} & \bm{$3.1$} & \bm{$-57.4$}\\
$Y$ Variance & $1.3$ & $8.7$ & $4.2$ & $7.6$ & $-0.1$\\
$Z$ Variance & $36.8$ & $12.6$ & $6.5$ & $14.0$ & $-4.3$\\
Determinant${{}}_{{XYZ}}$ & $21.0$ & $4.2$ & $3.7$ & $6.5$ & $-60.6$\\
Trace${{}}_{{XYZ}}$ & $18.2$ & $3.2$ & $1.9$ & $4.1$ & $-34.2$\\
$X$ Variance (robust) & $20.0$ & $3.4$ & $2.3$ & $4.1$ & $-63.4$\\
$Y$ Variance (robust) & $30.7$ & $14.7$ & $8.9$ & $12.1$ & $-5.2$\\
$Z$ Variance (robust) & $40.0$ & $12.2$ & $1.8$ & $11.8$ & $-18.3$\\
Determinant${{}}_{{XYZ}}$ (robust) & $21.3$ & $5.0$ & $3.4$ & $6.0$ & $-75.4$\\
Trace${{}}_{{XYZ}}$ (robust) & $20.8$ & $6.8$ & $3.5$ & $6.4$ & $-35.3$\\
\bm{$\xi^\prime$} \textbf{Variance} & \bm{$19.8$} & \bm{$1.5$} & \bm{$1.5$} & \bm{$2.5$} & \bm{$-71.1$}\\
$\eta^\prime$ Variance & $0.0$ & $6.2$ & $3.5$ & $7.2$ & $0.0$\\
$\zeta^\prime$ Variance & $36.3$ & $7.5$ & $2.0$ & $9.7$ & $-4.3$\\
Determinant${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ & $23.1$ & $3.8$ & $3.8$ & $6.3$ & $-60.5$\\
Trace${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ & $18.4$ & $3.2$ & $1.9$ & $4.0$ & $-34.0$\\
$\xi^\prime$ Variance (robust) & $20.0$ & $3.7$ & $2.1$ & $4.1$ & $-72.3$\\
$\eta^\prime$ Variance (robust) & $0.0$ & $12.5$ & $9.5$ & $11.3$ & $0.0$\\
$\zeta^\prime$ Variance (robust) & $40.0$ & $12.2$ & $1.8$ & $11.8$ & $-18.3$\\
Determinant${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ (robust) & $21.3$ & $4.9$ & $3.4$ & $6.0$ & $-75.3$\\
Trace${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ (robust) & $20.8$ & $6.8$ & $3.5$ & $6.3$ & $-35.1$\\
\sidehead{\textbf{Spatial--Kinematic Cross-Covariance Matrix}}
$X-U$ Cross-Covariance & $18.9$ & $2.3$ & $1.7$ & $3.1$ & $-75.8$\\
$Y-V$ Cross-Covariance & $0.0$ & $11.1$ & $4.9$ & $8.7$ & $0.0$\\
$Z-W$ Cross-Covariance & $35.7$ & $11.6$ & $8.7$ & $11.5$ & $-31.7$\\
Determinant${{}}_{{XUYVZW}}$ & $19.7$ & $8.1$ & $2.9$ & $8.4$ & $-63.5$\\
Trace${{}}_{{XUYVZW}}$ & $18.7$ & $3.2$ & $1.9$ & $4.1$ & $-74.0$\\
$X-U$ Cross-Covariance (robust) & $20.5$ & $2.9$ & $2.4$ & $4.0$ & $-65.8$\\
$Y-V$ Cross-Covariance (robust) & $34.2$ & $11.8$ & $9.6$ & $11.0$ & $-23.8$\\
$Z-W$ Cross-Covariance (robust) & $40.0$ & $11.9$ & $4.7$ & $11.8$ & $-13.8$\\
Determinant${{}}_{{XUYVZW}}$ (robust) & $25.1$ & $8.7$ & $2.9$ & $8.4$ & $-70.2$\\
Trace${{}}_{{XUYVZW}}$ (robust) & $15.7$ & $5.1$ & $2.7$ & $4.9$ & $-62.3$\\
$\xi^\prime-\dot{\xi}^\prime$ Cross-Covariance & $19.5$ & $1.7$ & $1.7$ & $2.9$ & $-83.4$\\
$\eta^\prime-\dot{\eta}^\prime$ Cross-Covariance & $0.2$ & $7.9$ & $2.7$ & $8.4$ & $-0.0$\\
$\zeta^\prime-\dot{\zeta}^\prime$ Cross-Covariance & $35.7$ & $11.6$ & $8.7$ & $11.5$ & $-31.7$\\
Determinant${{}}_{{\xi^\prime \dot{\xi}^\prime \eta^\prime \dot{\eta}^\prime \zeta^\prime \dot{\zeta}^\prime}}$ & $18.7$ & $8.4$ & $3.6$ & $8.6$ & $-48.4$\\
Trace${{}}_{{\xi^\prime \dot{\xi}^\prime \eta^\prime \dot{\eta}^\prime \zeta^\prime \dot{\zeta}^\prime}}$ & $20.5$ & $5.8$ & $2.2$ & $7.3$ & $-74.8$\\
$\xi^\prime-\dot{\xi}^\prime$ Cross-Covariance (robust) & $20.0$ & $6.4$ & $2.8$ & $4.9$ & $-75.6$\\
$\eta^\prime-\dot{\eta}^\prime$ Cross-Covariance (robust) & $6.6$ & $7.5$ & $3.1$ & $8.6$ & $-8.0$\\
$\zeta^\prime-\dot{\zeta}^\prime$ Cross-Covariance (robust) & $40.0$ & $12.0$ & $4.7$ & $11.8$ & $-13.8$\\
Determinant${{}}_{{\xi^\prime \dot{\xi}^\prime \eta^\prime \dot{\eta}^\prime \zeta^\prime \dot{\zeta}^\prime}}$ (robust) & $25.4$ & $8.2$ & $4.0$ & $9.2$ & $-60.4$\\
Trace${{}}_{{\xi^\prime \dot{\xi}^\prime \eta^\prime \dot{\eta}^\prime \zeta^\prime \dot{\zeta}^\prime}}$ (robust) & $29.0$ & $6.5$ & $6.3$ & $7.7$ & $-65.1$\\
\sidehead{\textbf{Median Absolute Deviation}}
MAD${{}}_{{X}}$ & $20.8$ & $5.3$ & $2.6$ & $5.5$ & $-64.3$\\
MAD${{}}_{{Y}}$ & $18.9$ & $10.8$ & $8.0$ & $10.7$ & $-2.8$\\
MAD${{}}_{{Z}}$ & $34.4$ & $13.6$ & $9.4$ & $13.7$ & $-10.8$\\
MAD${{}}_{{XYZ}}$ & $19.5$ & $7.1$ & $3.0$ & $7.0$ & $-36.0$\\
MAD${{}}_{{\xi^\prime}}$ & $19.6$ & $3.8$ & $1.5$ & $4.8$ & $-77.2$\\
MAD${{}}_{{\eta^\prime}}$ & $2.7$ & $11.7$ & $7.4$ & $12.7$ & $-3.3$\\
MAD${{}}_{{\zeta^\prime}}$ & $34.3$ & $13.6$ & $9.4$ & $13.1$ & $-10.8$\\
MAD${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ & $19.4$ & $7.1$ & $2.2$ & $7.5$ & $-34.7$\\
\sidehead{\textbf{Minimum Spanning Tree}}
MST${{}}_{{XYZ}}$ Mean & $24.3$ & $3.0$ & $2.9$ & $3.5$ & $-33.9$\\
MST${{}}_{{XYZ}}$ Mean (robust) & $18.7$ & $0.9$ & $2.9$ & $3.4$ & $-36.9$\\
MST${{}}_{{XYZ}}$ MAD & $22.6$ & $4.0$ & $5.7$ & $7.3$ & $-57.9$\\
MST${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ Mean & $24.3$ & $3.0$ & $2.9$ & $3.5$ & $-33.8$\\
MST${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ Mean (robust) & $18.7$ & $0.8$ & $2.9$ & $3.3$ & $-36.8$\\
MST${{}}_{{\xi^\prime \eta^\prime \zeta^\prime}}$ MAD & $22.6$ & $4.0$ & $5.7$ & $7.3$ & $-57.8$\\
\enddata
\tablecomments{Association size metrics are split across four categories based on the way they are computed: using the spatial covariance matrix, the spatial--kinematic cross-covariance matrix, the median absolute deviation (MAD), or the minimum spanning tree (MST). Both the $XYZ$ and the \xez\ coordinate systems are considered, as well as both empirical and robust covariance matrices metrics. Lines in bold characters are indicative of our most reliable size metrics. No correction to account for the effects of measurement errors was applied (see Section~\ref{sec:sensitivity_kinematic_errors}) (a)~The jackknife error is the error on the traceback age due to the sensitivity to sample definition, the measurement error is the error on the traceback age due to errors on astrometric and kinematic data, and the total error is computed with a Monte Carlo approach including both the jackknife and measurement errors (see Section~\ref{sec:error_traceback_age}). (b)~The contrast represent the change in association size at the epoch of minimal association size relative to the current-day epoch.}
\end{deluxetable*}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/trajectory_beta_pictoris.tex <==
\begin{figure}
 	\includegraphics{trajectory_beta_pictoris_fig.pdf}
 	\caption{Backward orbital integration of individual members of the core sample of \bpmg\ in \xez\ Galactic coordinates, back to $50$\,Myr into the past. Black circles indicate the members' positions at the current epoch, and blue circles indicate their positions at the epoch of minimal association size, as measured by the variance along the $\xi^\prime$-axis.\,This figure is adapted from Figure~3 of \cite{2020AA...642A.179M}.}
 	\label{fig:beta_pictoris_1}
\end{figure}

==> Addressing Systematics in the Dynamical Traceback Age of the Beta Pictoris Moving Group (with authors, ApJ)/trajectory_time_1x3_beta_pictoris.tex <==
\begin{figure}
    \includegraphics{trajectory_time_1x3_beta_pictoris_fig.pdf}
\end{figure}

\begin{figure}[t]
    \caption{Backward orbital integration of individual members of the core sample of \bpmg\ in \xez\ Galactic coordinates as a function of time, back to $50$\,Myr into the past. The average changes in position are the result of the average orbit in the Galaxy of members of the core sample of \bpmg, and the residual changes shown in all three panels are due to individual variations in $UVW$ space velocity among members. Black circles indicate the members' positions at the current epoch, and blue circles indicate their positions at the epoch of minimal association size, as measured by the variance along the $\xi^\prime$-, $\eta^\prime$- and $\zeta^\prime$-axes. The vertical dashed line represents the epoch of smallest spatial scatter using the same three association size metrics. The $\xi^\prime$ variance provides the most signal due to the greater velocity dispersion along this axis, whereas the $\zeta^\prime$ variance provides no useful data. This is an expected result of the Galactic orbits along this axis, which follow sinusoidal paths perpendicular to the Galactic plane.}
    \label{fig:beta_pictoris_2}
\end{figure}
